Industrial Experience Report on the Formal Specification of a Packet Filtering Language Using the K Framework

Many project-specific languages, including in particular filtering languages, are defined using non-formal specifications written in natural languages. This leads to ambiguities and errors in the specification of those languages. This paper reports on an industrial experiment on using a tool-supported language specification framework (K) for the formal specification of the syntax and semantics of a filtering language having a complexity similar to those of real-life projects. This experimentation aims at estimating, in a specific industrial setting, the difficulty and benefits of formally specifying a packet filtering language using a tool-supported formal approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{C. Dubois, P. Masci, D. M\'ery (Eds.): F-IDE 2016\\
EPTCS 240, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.240.3}{10.4204/EPTCS.240.3}}
\pdfoutput=1

